Braess's Paradox for Flows Over Time

We study the properties of Braess's paradox in the context of the model of congestion games with flow over time introduced by Koch and Skutella. We compare them to the well known properties of Braess's paradox for Wardrop's model of games with static flows. We show that there are networks which do not admit Braess's paradox in Wardrop's model, but which admit it in the model with flow over time. Moreover, there is a topology that admits a much more severe Braess's ratio for this model. Further, despite its symmetry for games with static flow, we show that Braess's paradox is not symmetric for flows over time. We illustrate that there are network topologies which exhibit Braess's paradox, but for which the transpose does not. Finally, we conjecture a necessary and sufficient condition of existence of Braess's paradox in a network, and prove the condition of existence of the paradox either in the network or in its transpose.

==> macros.tex <==
% vim: textwidth=78 foldmarker=<<<,>>> filetype=plaintex
%
% Lowlevel macros <<<

\makeatletter

\def\MyTokenizer#1#2#3{\@@MyTokenizer{#1}{#2}#3,\@nil}
\def\@@MyTokenizer#1#2#3,{#1{#2}{#3}\@ifnextchar\@nil{\@gobble}{\@@MyTokenizer{#1}{#2}}}

\def\MySet#1#2{\MyTokenizer{\@MySet}{#1}{#2}}
\def\@MySet#1#2{\@@MySet{#1}#2==\@nil}
\def\@@MySet#1#2=#3=#4\@nil{\@ifundefined{#1#2}{%
  \errmessage{Premenna "#1#2" neexistuje.}}{\expandafter\def\csname #1#2\endcsname{#3}}}

\def\MyDef#1#2{\MyTokenizer{\@MyDef}{#1}{#2}}
\def\@MyDef#1#2{\@@MyDef{#1}#2==\@nil}
\def\@@MyDef#1#2=#3=#4\@nil{\@ifundefined{#1#2}{%
  \expandafter\def\csname #1#2\endcsname{#3}}{\errmessage{Premenna "#1#2" uz existuje.}}}

\newcommand{\MyTuple}[2]{
  \begingroup
  \def\MyLocalComma{}
  \def\MyLocalGet##1##2{\MyLocalGetX{##1}##2==\@nil}
  \def\MyLocalGetX##1##2=##3=##4\@nil{\MyLocalComma\def\MyLocalComma{, }\csname##1##2\endcsname}
  \MyDef{MyLocalTuple}{#1}
  \ifx#2\undefined\else\MySet{MyLocalTuple}{#2}\fi
  (\MyTokenizer{\MyLocalGet}{MyLocalTuple}{#1})
  \endgroup
}

\let\MyOldColon=\colon
\def\colon{\ifmmode\MyOldColon\else{\rm:}\fi}

\def\myncarc{\pst@object{myncarc}}
\def\myncarc@i{\check@arrow{\myncarc@ii}}
\def\myncarc@ii#1#2{\nc@object{Open}{#1}{#2}{.5}{%
  yB yA sub xB xA sub \tx@Atan dup
  \psk@arcangleA\space add /AngleA ED
  \psk@arcangleB\space sub 180 add /AngleB ED
  \psk@ncurvB\space \psk@ncurvA\space
  GetEdgeA GetEdgeB xA1 xB1 sub yA1 yB1 sub Pyth 2 div dup 3 -1
  roll mul /ArmA ED mul /ArmB ED /ArmTypeA 0 def /ArmTypeB 0 def GetArmA
  GetArmB xA2 yA2 xA1 yA1 tx@Dict begin ArrowA end xB2 yB2 xB1 yB1 tx@Dict
  begin ArrowB end %curveto
  %
  \psk@arcangleA\space /Angle ED
  Angle 180 eq { 0 /Angle ED } if
  Angle 180 gt { Angle 360 sub /Angle ED } if
  /yB3 ED /xB3 ED currentpoint /yA3 ED /xA3 ED
  Angle 0 eq {
    xB3 yB3 moveto
    xA3 yA3 lineto
    0 /aA ED 0 /aB ED 0 /xS ED 0 /yS ED 0 /R ED
  } {
    /MyTan { dup sin exch cos div } def
    xA3 xB3 add 2 div Angle 90 eq { 0 } { yB3 yA3 sub 2 div Angle MyTan div } ifelse add /xS ED
    yA3 yB3 add 2 div Angle 90 eq { 0 } { xA3 xB3 sub 2 div Angle MyTan div } ifelse add /yS ED
    xA3 xS sub dup mul yA3 yS sub dup mul add sqrt /R ED
    yA3 yS sub xA3 xS sub atan /aA ED
    yB3 yS sub xB3 xS sub atan /aB ED
    xB3 yB3 moveto
    xS yS R aB aA Angle 0 lt { arcn } { arc } ifelse
  } ifelse
  %
  /LPutVar [ Angle xA3 yA3 xB3 yB3 aA aB xS yS R ] cvx def
  /LPutPos { LPutVar /R ED /yS ED /xS ED /aB ED /aA ED /yB3 ED /xB3 ED /yA3 ED /xA3 ED /Angle ED
    Angle 0 eq {
      xA3 xB3 xA3 sub t mul add /X ED
      yA3 yB3 yA3 sub t mul add /Y ED
      yB yA sub xB xA sub atan /NAngle ED
    } {
      Angle 2 mul 1 t sub mul aB add /aT ED
      gsave
      xB3 yB3 moveto
      xS yS R aB aT Angle 0 lt { arcn } { arc } ifelse
      currentpoint /Y ED /X ED
      grestore
      Y yS sub X xS sub atan 90 sub /NAngle ED
    } ifelse
  } def
  /HPutPos { LPutPos } def
  /VPutPos { LPutPos } def
}}

\def\mypcarc{\pst@object{mypcarc}}
\def\mypcarc@i{\pc@object\myncarc@ii}

\makeatother

% >>>
%
% Macros <<<

\newcommand{\MyNoSpellcheck}[1]{#1}

\ifx\keywords\undefined%
  \newenvironment{keywords}{\par\addvspace\baselineskip\noindent\textbf{Keywords:}\enspace\ignorespaces}{}%
\fi%

\setlength{\floatsep}{1em}
\setlength{\textfloatsep}{1em}
\setlength{\intextsep}{1em}
\setlength{\belowcaptionskip}{0pt}
\newenvironment{myfigure}{%
  \begin{figure}%
    \centering%
    \let\oldcaption=\caption%
    \let\oldlabel=\label%
    \renewcommand{\caption}[1]{\def\captionvalue{##1}}%
    \renewcommand{\label}[1]{\def\labelvalue{##1}}%
}{%
    \ifx\captionvalue\undefined\else%
      \begin{minipage}{0.8\textwidth}%
        \oldcaption{\captionvalue}%
        \ifx\labelvalue\undefined\else%
          \oldlabel{\labelvalue}%
        \fi%
      \end{minipage}%
    \fi%
  \end{figure}%
}

\newcommand{\MyArcPathX}[2]
{
  \addtocounter{MyArcPathCntr}{1}
  \ncput[npos=#2]{\dotnode{\varPrefix\the\value{MyArcPathCntr}}}
}
\newcommand{\MyArcPathY}[2]
{
  \addtocounter{MyArcPathCntr}{1}
  \myncarc[arcangle=(1;!#2 \varT\space sub #1 mul]{\varLast}{\varPrefix\the\value{MyArcPathCntr}}
  \edef\varLast{\varPrefix\the\value{MyArcPathCntr}}
  \def\varT{#2}
}
\newcounter{MyArcPathCntr}
\newcommand{\MyArcPath}[5][none]{{%[prefix]{angle}{A1}{A2}{t,...,t}
  \SpecialCoor
  \myncarc[arrows=-,linestyle=none,arcangle=#2]{#3}{#4}
  \setcounter{MyArcPathCntr}{0}
  \def\varPrefix{#1}
  \ifx#5\empty\else\MyTokenizer{\MyArcPathX}{}{#5}\fi
  \def\varLast{#3}
  \def\varT{0}
  \setcounter{MyArcPathCntr}{0}
  \ifx#5\empty\else\MyTokenizer{\MyArcPathY}{#2}{#5}\fi
  \myncarc[arcangle=(1;!1 \varT\space sub #2 mul)]{\varLast}{#4}
}}

\newcommand{\MyZigZagConnection}[3][none]{{% \MyZigZagConnection[prefix]{step}{arcs}
  \multido{\In=0+1,\Rpos=0.0+#2}{#3}{%
    \lput(\Rpos){\pnode{#1\In}}%
  }%
  \lput(1.0){\pnode{#1#3}}%
  \multido{\In=1+1,\Ilast=0+1}{#3}{%
    \ifodd\In\def\varAngle{33}\else\def\varAngle{-33}\fi%
    \myncarc[arcangle=\varAngle]{-}{#1\Ilast}{#1\In}%
  }%
}}%


% >>>
%
% Notations <<<

%%% Misc

\newcommand{\MyClass}[1]{\ensuremath{\mathcal{#1}}}
\newcommand{\dt}[1][t]{\ensuremath{\mathrm{d}#1}} % dx, dy, dt, etc. in integrals
\newcommand{\assign}{\ensuremath{\mathrel{\mathop:}=}} % :=

%%% Graphs

\newcommand{\MyGraphTranspose}[1]{\ensuremath{#1^T}}

\newcommand{\MyGraphOutlinks}{\ensuremath{\delta^{+}}}
\newcommand{\MyGraphOutlinksNode}[1]{\ensuremath{\MyGraphOutlinks_{#1}}}
\newcommand{\MyGraphInlinks}{\ensuremath{\delta^{-}}}
\newcommand{\MyGraphInlinksNode}[1]{\ensuremath{\MyGraphInlinks_{#1}}}

\newcommand{\MyPaths}{\ensuremath{P}}
\newcommand{\MyPathsFromTo}[2]{\ensuremath{\MyPaths_{{#1},{#2}}}}

%%% Congestion games

\newcommand{\CngInstanceName}[1]{\ensuremath{\mathrm{#1}}}

\newcommand{\CngSocialCost}[1][SC]{\ensuremath{\mathrm{#1}}}
\newcommand{\CngSocialCostNE}[1][SC]{\ensuremath{\CngSocialCost[#1]^*}}
\newcommand{\CngPoA}[1][\undefined]{\ensuremath{\mathrm{PoA}\ifx\undefined#1\else_{#1}\fi}}
\newcommand{\CngBraessRatio}[1][\undefined]{\ensuremath{\mathrm{BR}\ifx#1\undefined\else_{#1}\fi}}

%%% W-model

\newcommand{\WrdGraph}{\ensuremath{G}}
\newcommand{\WrdInstanceName}[1]{\CngInstanceName{#1}}

%%% FoT-model

\newcommand{\FoTGraph}{\ensuremath{G}}
\newcommand{\FoTCapacity}{\ensuremath{c}}
\newcommand{\FoTCapacityLink}[2][\FoTCapacity]{\ensuremath{#1_{#2}}}
\newcommand{\FoTTransitTime}{\ensuremath{\tau}}
\newcommand{\FoTTransitTimeLink}[2][\FoTTransitTime]{\ensuremath{#1_{#2}}}
\newcommand{\FoTSourceNode}{\ensuremath{s}}
\newcommand{\FoTSinkNode}{\ensuremath{t}}
\newcommand{\FoTSupply}{\ensuremath{d}}
\newcommand{\FoTInstance}[1][\undefined]{
  \MyTuple{G=\FoTGraph,c=\FoTCapacity,tau=\FoTTransitTime,
           s=\FoTSourceNode,t=\FoTSinkNode,d=\FoTSupply}{#1}}
\newcommand{\FoTInstanceName}[1]{\CngInstanceName{#1}}
\newcommand{\FoTAllInstances}{\MyClass{KS}}

\newcommand{\FoTST}[1][\FoTSinkNode]{\text{\FoTSourceNode-\ensuremath{#1}}}
\newcommand{\FoTPathsST}{\ensuremath{\MyPathsFromTo{\FoTSourceNode}{\FoTSinkNode}}}

\newcommand{\FoTFlow}{\ensuremath{f}}
\newcommand{\FoTInflow}[1][\FoTFlow]{\ensuremath{#1^{+}}}
\newcommand{\FoTOutflow}[1][\FoTFlow]{\ensuremath{#1^{-}}}
\newcommand{\FoTFlowLink}[2][\FoTFlow]{\ensuremath{#1_{#2}}}
\newcommand{\FoTInflowLink}[2][\FoTFlow]{\ensuremath{\FoTFlowLink[{\FoTInflow[#1]}]{#2}}}
\newcommand{\FoTOutflowLink}[2][\FoTFlow]{\ensuremath{\FoTFlowLink[{\FoTOutflow[#1]}]{#2}}}
\newcommand{\FoTCFlow}{\ensuremath{F}}
\newcommand{\FoTCInflow}[1][\FoTCFlow]{\ensuremath{#1^{+}}}
\newcommand{\FoTCOutflow}[1][\FoTCFlow]{\ensuremath{#1^{-}}}
\newcommand{\FoTCFlowLink}[2][\FoTCFlow]{\ensuremath{#1_{#2}}}
\newcommand{\FoTCInflowLink}[2][\FoTCFlow]{\ensuremath{\FoTCFlowLink[{\FoTCInflow[#1]}]{#2}}}
\newcommand{\FoTCOutflowLink}[2][\FoTCFlow]{\ensuremath{\FoTCFlowLink[{\FoTCOutflow[#1]}]{#2}}}

\newcommand{\FoTPathFlow}[2][\FoTFlow]{\ensuremath{#1^{#2}}}

\newcommand{\FoTSinkFlow}{\ensuremath{\gamma}}
\newcommand{\FoTCSinkFlow}{\ensuremath{\Gamma}}

\newcommand{\FoTWaitingTime}{\ensuremath{q}}
\newcommand{\FoTWaitingTimeLink}[1]{\ensuremath{\FoTWaitingTime_{#1}}}

\newcommand{\FoTLabelFunc}{\ensuremath{\ell}}
\newcommand{\FoTLabelFuncNode}[1]{\ensuremath{\FoTLabelFunc_{#1}}}

\newcommand{\FoTPrice}{\ensuremath{\lambda}}
\newcommand{\FoTPriceLink}[1]{\ensuremath{\FoTPrice_{#1}}}
\newcommand{\FoTPriceNode}[1]{\ensuremath{\FoTPrice_{#1}}}
\newcommand{\FoTPricePath}[1]{\ensuremath{\FoTPrice_{#1}}}

\newcommand{\FoTCMAX}{\ensuremath{\CngSocialCost[CMAX]}}
\newcommand{\FoTCAVG}{\ensuremath{\CngSocialCost[CAVG]}}
\newcommand{\FoTPoAcmax}{\ensuremath{\CngPoA[\FoTCMAX]}}
\newcommand{\FoTPoAcavg}{\ensuremath{\CngPoA[\FoTCAVG]}}
\newcommand{\FoTPoAevac}{\ensuremath{\CngPoA[\mathit{evac}]}}
\newcommand{\FoTPoAtime}{\ensuremath{\CngPoA[\mathit{time}]}}

% >>>
%


